Deterministic Parikh automata on infinite words

Various variants of Parikh automata on infinite words have recently been introduced in the literature. However, with some exceptions only their non-deterministic versions have been considered. In this paper we study the deterministic versions of all variants of Parikh automata on infinite words that have not yet been studied. We compare the expressiveness of the deterministic models and investigate their closure properties and decision problems with applications to model checking. The model of deterministic limit Parikh automata turns out to be most interesting, as it is the only deterministic Parikh model generalizing the $\omega$-regular languages, the only deterministic Parikh model closed under the Boolean operations and the only deterministic Parikh model for which all common decision problems are decidable.

==> review.tex <==
---------------------- REVIEW 1 --------------------

Related work: the authors could be more generous with citations, specially of the models or logics that they mention. For instance, Büchi VASS, counting MSO, Boolean algebra with Presburger arithmetic, or Ramsey quantifiers, where works dealing with these concepts are cited but the seminal works are not.

Preliminaries:

Parikh automata on infinite words:

There are four formal issues with this section.

First, why is it not included in the preliminaries? If the material in reference 11 has already been accepted to CSL then this should probably go in the preliminaries.

Second, there is a lot of duplication. Each definition of an automata model is followed by an equation where the right hand side is identical for each instance. I am not sure this contributes positively to the readability of the paper. Perhaps some kind of illustration of the acceptance condition can help. Then instead of the equation, one can say “the set of words accepted by A under this criterion is denoted by …”.

Third, the paragraph starting in line 340 could be improved for the benefit of the reader. It appears to me that the crucial point is to clarify to the reader whether the completeness assumption has some cost. At the moment, this is phrased in the positive “allows to express additional safety conditions”. Is that not good? How can then the restriction be considered “pure”?. This point should be clarified. Then the paper should clarify which models can be completed. I’m assuming they mean models (1), (3), (4). Given that they used an enumeration of the models  this is the perfect place to use it. It is also important to clarify whether the completeness assumption has some penalty for these models. At the moment, it could be inferred that not, but it would be useful to explicitly state it.

Four, the last paragraph relies on 11, I’m assuming this is published in CSL and thus I do not have to check the validity of the claims.

Expressiveness:

There are a variety of methodological issues.

When you explain the you give the strongest separation I believe I understand what is meant, but perhaps a formal statement of this claim should be made. Or even better, you could show the expressivity inclusions in a graph, then the reader can go to the graph and check that indeed you always show the non-inclusions between the upper-bound and the lower-bound of two distinct chains of inclusions. This would complement the informative tables of the introduction.

You also say that you have an abuse of notation. Maybe just say that you use such notation to indicate such property, I do not think the two interpretations of inclusion are going to be mixed up.

In the proof of Lemma 4.2, either give the specific reference to the result in 22, this can be done for instance in latex with \cite[Theorem~3]{reference_22} or do one example from the four non-inclusions that you claim.
In the proof of Lemma 4.3 you have a forward reference to Lemma 4.5, is it really necessary given that the proof of that lemma is roughly 3 lines long? I would rethink the structure of the presentation. You also have a backward reference to “the previous proof” which I believe is Lemma 4.2, maybe it is better to use the numbering..

In Section 4.2, it would be beneficial to quote the specific results from references 11 and 12 that are needed in the form mentioned before.

In Section 4.3, I would omit references to arXiv versions since these are not peer reviewed. You also use the abbreviation Reach PA, then in line 558/559 you use a dot to signal the abbreviation “reach-reg.”. So maybe an intermediate solution is to write the full name in the title of the Sections, e.g. “Deterministic Reachability PA” and if there is lack of space in the statements of lemmas, just write “Deterministic reach”.” PA …” with the explicit dot signalling the abbreviation.

Overall my most important recommendation for this section would be to include a diagram of the resulting inclusions.

Closure properties:

There are some minor problems and some suggestions I think that would really improve the contribution.

Regarding the minor problems, these are in the same vein as before. For instance, in line 670/671 you cite reference 13 which is a survey, this is fine, but shouldn’t credit be given to the people that first proved closure under complement of semi-linear sets. One would have to check but I guess maybe Ginsburg and Spanier did so. Citing both works is also fine. Again, there is a weird spelling in line 728/729 where P appears with a tilde, the abbreviation of reach-reg. As discussed before, it is fine since it is there for fitting into the column size I guess. Then in line 829, it should be made explicit that “The authors…” means “The authors of [11]...”.

My major concern then is on the ordering of the results. It seems to me that the results of Section 5 only depend on Section 4 for the languages that witness the different properties (which were introduced in Section 4). On the other hand, the paragraph starting in 823 makes an important observation with respect to Section 4, they show that the expressivity is reduced by passing to the deterministic model. Thus, I think the authors should seriously think about changing the order of Section 5 and Section 4. This paragraph would then be moved to the expressivity section and would be used to complete a diagram of the expressivity of the different models. The paragraph would also be reformulated as a corollary of the closure properties. Putting an explicit corollary allows future research to reference that particular result instead of having the risk of this statement becoming a “folklore result”.

Decision Problems and Model Checking:

The same general remarks apply to this section. Otherwise, maybe clarify at the beginning of Section 6.1 why you study these decision problems and not others. I believe this is because you use those in Section 6.2?
The other remark is that I do not see a comment on why the universality problem is not given more precise complexity bounds (table 2 only lists decidability for this case).

Conclusion:

The conclusion raises open questions in the area of synthesis and regular separability which will stimulate research in the area. I am missing some further recapitulation of the results of the paper. In particular, it seems that the expressivity results are not mentioned?

References:

The state of the references fades the shine of the paper. One paper includes a doi while the others don’t. Some papers like reference eleven are not given full details (I checked online and this does seem to be published now in CSL). The references are given in two columns, when they could be given in a single column. Please address these issues in the final version. A reference manager like Zotero or Mendeley should help in avoiding these problems.


----------------------- REVIEW 2 ---------------------
SUBMISSION: 75
TITLE: Deterministic Parikh automata on infinite words
AUTHORS: Mario Grobler and Sebastian Siebertz

----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
Summary:

This paper builds upon the recent work of Guha et al. [12] and Grobler et al [11] to study Parikh automata (PA) over infinite words, in particular, deterministic PA over infinite words. The paper discusses several models of Parikh automata over infinite words that were introduced in Guha et al [12] and Grobler et al [11] in Section 3. Section 4 compares the expressiveness of these PA models while Section 5 studies closure under Boolean operations for the deterministic version of the models that were introduced in [11]. Section 6.1 includes results on decision problems like non-emptiness, universality, and membership problems for the models introduced by Grobler et al in [11]. Section 6.2 finally contains the study of existential model checking and universal model checking.


Evaluation:

While the paper studies a nice and almost complete set of automata theoretic questions for various deterministic versions of Parikh automata over infinite words that were recently introduced in [11] and [12], the results are largely adapted from previous works and often follow easily using known and similar techniques that are used in [12]. Besides, at a few places, for example, lemmas 4.3 to 4.5 (see below), the paper proves a few results which already exist in [12]. The paper is mostly well written with the exception of Section 6.2 where some details are missing or vague and some explanations require to be improved. While the paper captures a nice set of results, the technical novelty of the work is rather limited.


Questions and comments:

Table 3: Do the crosses and tick denote undecidable and decidable respectively?

L 182: languages --> language
In Section 4, it might be worth mentioning how deterministic Reach PA and deterministic Buchi PA compare. My understanding is that they are incomparable. However, this needs a proof. The language L considered in Lemma 4.7 may help to show that it cannot be accepted by a deterministic Buchi PA.

459-460: safety PA do not recognize the language {a,b}^omega \ a^omega: Could you state where in [12] this result appears as claimed?

L 461- 463: Finally, dually ... we can show: The result appears in the proof of Thm 3 (BPA \not \subseteq CPA) in the arXiv version of [12]. However this has not been cited and claimed as a new proof.

Cor 4.4, L 471: Det Buchi \not subseteq Det safety, Det co-Buchi also appear in the proof of Thm 3 in the arXiv version of [12]. However this has not been cited and claimed as a new proof.

Lemma 4.5: The idea of the proof already exists in the proof of Thm 3 in the arXiv version of [12] using the notion of FC-prefixes.

L 558: showing that the --> showing that
L 576-578 {a^nb^n | n>0}^\omega cannot be recognized by Buch PA: This requires a proof.

Lemma 4.14: It is not clear why the proof is identical to Lemma 4.7 since moving once does not suffice. One may need to move infixes infinitely many times.  A similar idea exists in the proofs of Thm 1 and Thm 6 in [12].

Lemma 5.1: Can there be an alternative/simpler proof using Presburger arithmetic?

L 662: Typo: \mathfrak{A}_1 --> \mathfrak{A}
L 694, 705: An example would help here.
L 740: L is not defined.
L 814: c^{n_1-i_1} --> c^{i_1-n_1}
L 815: c^{n_2-i_2} --> c^{i_2-n_2}
L 865: Add the original citations which can be found in reference [13].
L 894: be --> by

The overall readability of Sec 6.2 needs to be improved. The proofs of Lemma 6.9 (the part starting from L 1066) and Lemma 6.10 are difficult to follow. In the proof of Lemma 6.10, more intuitive description rather than the formal definition would have been useful. How does Corollary 6.11 for det limit PA and det strong reset PA follow from the proof of Lemma 6.10? The proof of Lemma 6.13 is also vague at some places.

L 954-955: as a PA: Do you mean reach PA on infinite words?
Proof of Lemma 6.8 and 6.9: The input automata are A and B and the product automaton is also called A which causes confusion at times.

L 1038: "Hardness is obvious": Add that it follows trivially from the emptiness problem.

L 1070: Two achieve: To achieve
L 1077: To which copy does the final state (p_{\ell+1}, q_{\ell+1}) belong to? This information should be part of the final state.
L 1101: Semantics of Z-VASS_k^{nz} is not defined. Please add what the k stands for (I had to check reference 15 to understand the definition.).

L 1305-1307: Could you elaborate on the statement 'To be able to perform the correct check ...'.? How is the fifth counter used?
L 1349-1351: What are the accepting states and what is the associated semilinear set C?


----------------------- REVIEW 3 ---------------------
SUBMISSION: 75
TITLE: Deterministic Parikh automata on infinite words
AUTHORS: Mario Grobler and Sebastian Siebertz

----------- Overall evaluation -----------
SCORE: 1 (weak accept)
----- TEXT:
Parikh automata extend the classical model of finite-state automata with weights on transitions and a semilinear set. A word is accepted by a Parikh automaton if there is an execution of the finite-state automaton on the given word which ends in a final state and the accumulated weights belongs to the semi-linear set. This model is well-studied and has been extended to infinite words with various acceptance conditions. This paper focuses on the subclasses of deterministic Parikh automata over infinite-words. First, the paper studies the closure properties of different classes of deterministic Parikh automata. Next, the authors consider a variety of decision problems, including emptiness, universality, and model checking.

This paper considers interesting and relevant problems. The paper is mostly well-written and easy to follow. The authors present a nice collection of results about deterministic Parikh automata over infinite words. The proofs seem to be correct (but not technically deep). The main drawback of the paper is that most of the results are not difficult to obtain. Most of the proofs are straightforward and follow standard techniques. I suppose that this can be compensated by the exhaustive study done by the authors on the different closure properties and decision problems of the classes of deterministic Parikh automata.

Overall, the paper contains a collection of nice and interesting results and fits well within the LICS topics. It advances the state of the art (even if the complexity of some of the results presented remains open).
